Inf-sup stability of the trace P2-P1 Taylor-Hood elements for surface PDEs

The paper studies a geometrically unfitted finite element method (FEM), known as trace FEM or cut FEM, for the numerical solution of the Stokes system posed on a closed smooth surface. A trace FEM based on standard Taylor-Hood (continuous P2-P1) bulk elements is proposed. A so-called volume normal derivative stabilization, known from the literature on trace FEM, is an essential ingredient of this method. The key result proved in the paper is an inf-sup stability of the trace P2-P1 finite element pair, with the stability constant uniformly bounded with respect to the discretization parameter and the position of the surface in the bulk mesh. Optimal order convergence of a consistent variant of the finite element method follows from this new stability result and interpolation properties of the trace FEM. Properties of the method are illustrated with numerical examples.

==> tab/sphere_2_P2P1_patchnormals=0_shift=0.0_form=consistent_m=12_rhofac=1_rhopow=-1_conv_table.tex <==
$8.3\times	10^{-1}$	&	$1.2$	&	$\text{}$	&	$4.8\times	10^{-1}$	&	$\text{}$	&	$4.2\times	10^{-1}$	&	$\text{}$	\\ \hline
$4.2\times	10^{-1}$	&	$3.7\times	10^{-1}$	&	$1.8$	&	$6.1\times	10^{-2}$	&	$3.$	&	$1.1\times	10^{-1}$	&	$2.$	\\ \hline
$2.1\times	10^{-1}$	&	$9.2\times	10^{-2}$	&	$2.$	&	$5.8\times	10^{-3}$	&	$3.4$	&	$2.5\times	10^{-2}$	&	$2.1$	\\ \hline
$1.\times	10^{-1}$	&	$2.2\times	10^{-2}$	&	$2.1$	&	$5.6\times	10^{-4}$	&	$3.4$	&	$6.3\times	10^{-3}$	&	$2.$	\\ \hline
$5.2\times	10^{-2}$	&	$5.4\times	10^{-3}$	&	$2.$	&	$5.2\times	10^{-5}$	&	$3.4$	&	$1.7\times	10^{-3}$	&	$1.8$	\\ \hline
$2.6\times	10^{-2}$	&	$1.4\times	10^{-3}$	&	$2.$	&	$5.4\times	10^{-6}$	&	$3.3$	&	$5.3\times	10^{-4}$	&	$1.7$	\\ \hline
$1.3\times	10^{-2}$	&	$3.5\times	10^{-4}$	&	$2.$	&	$6.9\times	10^{-7}$	&	$3.$	&	$1.8\times	10^{-4}$	&	$1.6$	\\ \hline

==> tab/sphere_2_P2P1_patchnormals=0_shift=0.0_form=consistent_m=12_rhofac=1_rhopow=-1_iters_table.tex <==
$8.33\times	10^{-1}$	&	$3.4\times	10^{-1}$	&	$\text{}$	&	$26$	&	$7.3\times	10^{-9}$	\\ \hline
$4.17\times	10^{-1}$	&	$5.3\times	10^{-2}$	&	$2.7$	&	$33$	&	$4.8\times	10^{-9}$	\\ \hline
$2.08\times	10^{-1}$	&	$4.9\times	10^{-3}$	&	$3.4$	&	$31$	&	$6.\times	10^{-9}$	\\ \hline
$1.04\times	10^{-1}$	&	$5.\times	10^{-4}$	&	$3.3$	&	$27$	&	$8.3\times	10^{-9}$	\\ \hline
$5.21\times	10^{-2}$	&	$4.9\times	10^{-5}$	&	$3.4$	&	$26$	&	$8.6\times	10^{-9}$	\\ \hline
$2.6\times	10^{-2}$	&	$5.\times	10^{-6}$	&	$3.3$	&	$26$	&	$7.5\times	10^{-9}$	\\ \hline
$1.3\times	10^{-2}$	&	$5.9\times	10^{-7}$	&	$3.1$	&	$34$	&	$8.\times	10^{-9}$	\\ \hline

==> tab/sphere_2_P2P1_patchnormals=0_shift=0.0_form=inconsistent_m=12_rhofac=1_rhopow=1_conv_table.tex <==
$8.3\times	10^{-1}$	&	$3.$	&	$\text{}$	&	$1.8$	&	$\text{}$	&	$2.1$	&	$\text{}$	\\ \hline
$4.2\times	10^{-1}$	&	$1.8$	&	$7.4\times	10^{-1}$	&	$9.1\times	10^{-1}$	&	$9.7\times	10^{-1}$	&	$1.7$	&	$2.7\times	10^{-1}$	\\ \hline
$2.1\times	10^{-1}$	&	$7.\times	10^{-1}$	&	$1.4$	&	$3.4\times	10^{-1}$	&	$1.4$	&	$6.9\times	10^{-1}$	&	$1.3$	\\ \hline
$1.\times	10^{-1}$	&	$2.\times	10^{-1}$	&	$1.8$	&	$9.9\times	10^{-2}$	&	$1.8$	&	$2.\times	10^{-1}$	&	$1.8$	\\ \hline
$5.2\times	10^{-2}$	&	$5.2\times	10^{-2}$	&	$1.9$	&	$2.6\times	10^{-2}$	&	$1.9$	&	$5.2\times	10^{-2}$	&	$1.9$	\\ \hline
$2.6\times	10^{-2}$	&	$1.3\times	10^{-2}$	&	$2.$	&	$6.5\times	10^{-3}$	&	$2.$	&	$1.3\times	10^{-2}$	&	$2.$	\\ \hline
$1.3\times	10^{-2}$	&	$3.3\times	10^{-3}$	&	$2.$	&	$1.6\times	10^{-3}$	&	$2.$	&	$3.3\times	10^{-3}$	&	$2.$	\\ \hline

==> tab/sphere_2_P2P1_patchnormals=0_shift=0.0_form=inconsistent_m=12_rhofac=1_rhopow=1_iters_table.tex <==
$8.33\times	10^{-1}$	&	$1.8$	&	$\text{}$	&	$24$	&	$6.2\times	10^{-9}$	\\ \hline
$4.17\times	10^{-1}$	&	$9.2\times	10^{-1}$	&	$9.4\times	10^{-1}$	&	$31$	&	$5.4\times	10^{-9}$	\\ \hline
$2.08\times	10^{-1}$	&	$3.5\times	10^{-1}$	&	$1.4$	&	$30$	&	$9.8\times	10^{-9}$	\\ \hline
$1.04\times	10^{-1}$	&	$9.9\times	10^{-2}$	&	$1.8$	&	$27$	&	$7.8\times	10^{-9}$	\\ \hline
$5.21\times	10^{-2}$	&	$2.6\times	10^{-2}$	&	$1.9$	&	$26$	&	$8.3\times	10^{-9}$	\\ \hline
$2.6\times	10^{-2}$	&	$6.5\times	10^{-3}$	&	$2.$	&	$26$	&	$9.6\times	10^{-9}$	\\ \hline
$1.3\times	10^{-2}$	&	$1.6\times	10^{-3}$	&	$2.$	&	$35$	&	$7.\times	10^{-9}$	\\ \hline
